A Mechanistic View of Authority Hierarchy in LLM Sycophancy

Authority bias poses a critical safety concern in language models: models systematically prioritize social cues from authority figures over factual consistency, swaying their answers based on source credibility rather than evidence. We mechanistically investigate this phenomenon using a controlled medical QA setting, where hints suggesting incorrect answers are attributed to personas of varying expertise. Across Llama-3.1-8B, Qwen3-8B, and Gemma-2-9B, we find that models respond in a graded manner proportional to perceived authority, a hierarchy that is never explicitly prompted but emerges from training. Logit lens analysis and linear/non-linear probing localize this effect to a critical late layer where correct answer representations are actively erased, an erasure that scales with authority level, resists mean vector intervention, and is only partially reversible through chain-of-thought reasoning. Our findings suggest that authority-induced sycophancy is not a surface-level output bias but mechanistic knowledge erasure, a precise, layer-localized overwriting of correct internal representations by high-status authority signals.

==> methods.tex <==

\section{Methods}
We can put the methods and results separate if needed (may be for EMLP audience)
\subsection{Activation Analysis}




\subsection{Linear Projection}


\subsection{Linear Probing}

Write about the technique, model layers etc

\textbf{Show the 4 experts graph together up and down - resisted and flipped}



The finding is that traditionally, we would expect a model is sycophantic when the model knows the answer, but reverts to the given suggestion, but we can argue that, in this case that is not happening, ie, the knowledge itself is completely getting removed somehow to a point where it is not recoverable. Now, if this is true, we can claim that in such cases, even cot should not be able to recover the correct answer. 

When you compare this with the logit lens of this same (data, model), we can see that the activations no longer have the correct information inside them after layer 28.





